A Novel Data Augmentation Technique for Out-of-Distribution Sample Detection using Compounded Corruptions

Modern deep neural network models are known to erroneously classify out-of-distribution (OOD) test data into one of the in-distribution (ID) training classes with high confidence. This can have disastrous consequences for safety-critical applications. A popular mitigation strategy is to train a separate classifier that can detect such OOD samples at the test time. In most practical settings OOD examples are not known at the train time, and hence a key question is: how to augment the ID data with synthetic OOD samples for training such an OOD detector? In this paper, we propose a novel Compounded Corruption technique for the OOD data augmentation termed CnC. One of the major advantages of CnC is that it does not require any hold-out data apart from the training set. Further, unlike current state-of-the-art (SOTA) techniques, CnC does not require backpropagation or ensembling at the test time, making our method much faster at inference. Our extensive comparison with 20 methods from the major conferences in last 4 years show that a model trained using CnC based data augmentation, significantly outperforms SOTA, both in terms of OOD detection accuracy as well as inference time. We include a detailed post-hoc analysis to investigate the reasons for the success of our method and identify higher relative entropy and diversity of CnC samples as probable causes. We also provide theoretical insights via a piece-wise decomposition analysis on a two-dimensional dataset to reveal (visually and quantitatively) that our approach leads to a tighter boundary around ID classes, leading to better detection of OOD samples. Source code link: https://github.com/cnc-ood

==> macros-and-includes.tex <==
\usepackage{multirow,epsfig,pdflscape,graphicx,amsmath,amssymb}
\usepackage{float}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{graphicx,textcomp}
\usepackage{mathrsfs}
\usepackage{empheq}
\usepackage{amssymb}
\usepackage{rotating}
%\usepackage{subcaption}
\usepackage{caption}
\def\etal{{et al.\xspace}}
%\usepackage{subcaption}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs} 
\usepackage[dvipsnames]{xcolor}
% professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}
%\usepackage[noadjust]{cite}
\usepackage{array, tabularx,  ragged2e,  booktabs}

%\usepackage[font=small,skip=5pt,belowskip=0pt]{caption}
%\setlength{\textfloatsep}{5pt}

\usepackage{longtable}
\usepackage{textcomp}
\usepackage{siunitx}
%\usepackage{subfig}
\usepackage{array}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
%\usepackage{algorithm} % http://ctan.org/pkg/algorithms
\usepackage[noend]{algpseudocode} % http://ctan.org/pkg/algorithmicx

\usepackage{algpseudocode}
\usepackage{romannum}
%\usepackage{amsthm}
\usepackage{graphicx}
\usepackage{xcolor}

\usepackage{algorithmicx}
%\usepackage{subcaption}
%\usepackage[usenames,dvipsnames]{xcolor}
%\usepackage{times}
\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{appendix}
\usepackage{etoolbox}
\usepackage{soul}
\usepackage{tabularx}
\usepackage{rotating,comment}
\usepackage[outercaption]{sidecap}  
\usepackage{wrapfig}
\usepackage{subfigure}
%\usepackage{subfig}
\renewcommand{\restriction}{\mathord{\upharpoonright}}



\usepackage[inline]{enumitem}

%\newcommand\figref[1]{Figure~\ref{#1}}
%\newcommand\tabref[1]{Table~\ref{#1}}

\usepackage[pagebackref,breaklinks,colorlinks,bookmarks=false]{hyperref}
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}
\crefname{figure}{Fig.}{Figs.}

\BeforeBeginEnvironment{appendices}{\clearpage}

%\newcolumntype{Y}{>{\centering\arraybackslash}X}
\def\lce{{\mathcal{L}_{\rm CE}}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\minimize}{minimize}



\definecolor{todocolor}{RGB}{200,120,120}
\sethlcolor{todocolor}
\newcommand{\todo}[1]{\textcolor{black}{\hl{#1}}}

%\newcommand{\figref}[1]{Fig.~\ref{#1}}
%\newcommand{\secref}[1]{Sec.~\ref{#1}}
\usepackage{graphicx} 
%\usepackage[showframe]{geometry}

\def\X{{\mathcal{X}}}
\def\Y{{\mathcal{Y}}}
\def\D{{\mathcal{D}}}

\def\dP{{\mathbb{P}}}
\def\cP{{\mathcal{P}}}
\def\cQ{{\mathcal{Q}}}
\def\cM{{\mathcal{M}}}

\def\real{{\mathbb{R}}}

%\def\ood{\textsc{ood}\xspace}
%\def\iid{\textsc{iid}\xspace}
%\def\id{\textsc{id}\xspace}
%\def\sota{\textsc{sota}\xspace}
%\def\dnn{\textsc{dnn}\xspace}


\def\xt{{\Tilde{x}}}
\def\yt{{\Tilde{y}}}
\def\hbe{{\mathbf{\emph{h}}}}
\def\HC{{\mathcal{H}}}

%\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
%\newcolumntype{N}{@{}m{0pt}@{}@{}}

%\newcommand{\myfirstpara}[1]{\noindent \textbf{#1:}}
%\newcommand{\mypara}[1]{\vspace{0.2em} \myfirstpara{#1}}

\newcommand{\multilineC}[1]{\begin{tabular}[b]{@{}c@{}}#1\end{tabular}}
\newcommand{\multilineCB}[1]{\textbf{\multilineC{#1}}}
\newcommand{\vertext}[1]{\begin{turn}{90} {#1} \end{turn}}

%\fboxsep=0.2mm%padding thickness
%\fboxrule=0.02pt%border thickness

\graphicspath{{figs-main/}}
\graphicspath{{./figs/}}
\usepackage{wrapfig,lipsum,booktabs}



==> old-intuition-subsection-unused.tex <==

\subsection{Intuition for Compounded Corruptions}
%
We leverage proxy \ood data to improve \ood detection accuracy \textcolor{red}{with no or negligible compromise on ID accuracy}. Since there is no principled way to generate samples that span the entire \ood space which is practically an infinite set, we come up with a strategy to generate proxy \ood data by applying a combination of CutMix \cite{yun2019cutmix} and corruptions\cite{hendrycks2018benchmarking} on training image set. While we empirically validate in experiments section that CnC works better than the state of the art, we have \textcolor{red}{$3$} hypotheses,\textcolor{red}{\textbf{(H1, H2, H3)}}, on why it works better. 

\mypara{H1: Perturbing object and its context}
%
Under the compositional model for image classification, the image can be broadly assumed to be made up of two components, a \emph{foreground} consisting of salient object determining the class label of the image, and a \emph{background} consisting of the context in which the object appears. Changes in the foreground, background or their co-occurrence can make an image an \ood sample. For eg., a foreground object consisting of half cat, and half dog is clearly \ood; so is a fish on a chair.


% Rahul : If the end goal is to classify the foreground, why does it matter that the fish is on a sofa? Should it not still be classified as a fish instead of OOD? More importantly, what if you change the background of a dog so that the dog is sitting on a sofa (which is OK for a dog)?

%Similarly a dog appearing on half grass, and half sofa is also an \ood sample, as well as a dog floating in sea, or a fish on a sofa. 
Intuitively CutMix allows us to generate samples with  invalid configurations, thereby allowing a network to learn correct shape as well as context of the \id object. The other criterion for a valid object to be detected as \id is its visual appearance, determined by the texture, contrast, and illumination. For example, a green dog or \textcolor{red}{any elastically transformed object} could be treated as an \ood. This is where the role of corruptions which disturb the visual appearance and help network learn what is not a valid \id sample. So the proposed corruption over CutMix style of creating \ood samples allows us to semantically span a large space of \ood examples. 



%Rahul : Fig 3 doesn't clearly support your arguments. You'll have to point out that almost all corrupted images are almost on top of the ID samples. Odd that the corrputed images also seem to be staying in the convex hull of the ID data, why is that? Also the Cut-and-Mix images don't seem to lie in line segments between pairs of ID samples either, despite what you say in Sec 5.2, they are more spread out.

%\mypara{Decomposition using piecewise approximations}
%\cite{jordan2019provable}

\mypara{H2: Diversity and Entropy}
%
Our second hypothesis regarding CnC performance is inspired by learning theory. We observe that CutMix not only generates an \ood image as convex combination of the two images belonging to separate \id classes, but the embedding vector of the generated sample is also approximately convex combination of the embedding vectors of the corresponding images from the visualisations~\cite{Pang*2020Mixup, zhang2017mixup} (see suppl for empirical support). Hence, generating samples using CutMix allows us to generate samples which are diverse not only in the RGB space, but in the embedding space as well. \cref{fig:umap} shows a UMAP ~\cite{mcinnes2018umap} visualization of data generated data points. UMAP preserves the global structure in the final projection in comparison to t-SNE \cite{van2008visualizing}, the inter-cluster relations in UMAP are potentially more meaningful than in t-SNE despite of data warping in the projection space, hence used in our visualization. 

%of why CnC works better than the state of the art is inspired from the learning theory. 
%It has been shown that the neural networks behave linearly in the local neighborhoods \cite{goodfellow2014explaining}. 
% Rahul : "It has been shown that neural networks behave linearly in the local neighborhoods" So what? Any differentiable function behaves linearly in a local neighbourhood.


Impact of diversity on the improved learning of machine learning models is well studied in the literature \cite{Gong_2019}. We use data diversity \cite{zhang2019active, Gong_2019} to quantitatively measure the diversity of generated samples from various techniques. Data diversity is defined as the normalised minimum distance between any two \ood points, $x_i$ and $x_j$ in the embedding space. We use euclidean distance as the distance metric for calculating diversity in K dimensional space. \cref{tab:diversity_entropy} shows the correlation between diversity and \ood detection performance of various approaches. %Our technique has maximum diversity as well as best \ood detection performance. 

We observe that the probability vector generated by say a K classifier on the CutMix generated samples may still have low entropy. For example, a sample generated by a convex combination of a cat and a dog image, may generate a probability vector giving 0.5 to cat, and 0.5 to dog, a low entropy vector compared to uniform distribution on a 10 class classifier. Similar to diversity, high entropy in the training samples has also been proposed as a metric to measure the usefulness of a sample to train a machine learning model \cite{Gong_2019}. Lee \etal\cite{lee2017training} include additional terms in the training objective that force the \ood points to have maximum entropy. This is achieved through  minimizing the KL divergence between the model generated probabilities on OOD samples to uniform distribution. Similarly, Hendrycks \etal \cite{hendrycks2018deep} also force the \ood samples to have uniform distribution. Hence, role of a corruption in the proposed approach is to convert the diverse samples from the CutMix in a way such that they generate a high entropy probability vector when passed through a pre-trained K-class classifier. 
%We benchmark various \ood sample generation techniques with the accuracy obtained by the \ood detector when trained with such samples. 
We empirically show that diversity and entropy of the generated samples is a good indicator of their suitability for training an \ood detector.



==> pseudocode.tex <==
\begin{algorithm}
	%\algsetup{linenosize=\tiny}
	\scriptsize %\small, \footnotesize, \scriptsize, or \tiny
	\label{algo_Rasha}
	\SetKwInput{KwInput}{Inputs}                % Set the Input
	\SetKwInput{KwOutput}{Output}  
	\SetKwInput{KwLoss}{Loss}  
	\DontPrintSemicolon
	\LinesNotNumbered
	\KwInput{
		$\D^\text{train}_\text{in}$  \tcp*{Train Set} 
		${f_{\theta}^+}$, $m$  \tcp*{Model, Number of epochs}
		$\mathcal{O}$ = \{contrast, $\cdots$, frost\} \tcp*{Corruption set}
		$\mathcal{S}$ = \{1, 2, 3, 4, 5\} \tcp*{Severity}
		$K+1$ \tcp*{Number of Classes}
	}
	\KwOutput{Trained Model $F^+$}
	%\tcp{\ood Data Generation}
	\SetKwFunction{FSum}{CnCDataGen} %\tcp*{\ood Data Generation} 
	
	\SetKwProg{Fn}{Function}{}{}
	\Fn{\FSum{X$_{ID}$}}{
		X$_\text{pbcc} \leftarrow$ Apply PBCC on X$_{ID}$ as described in Sec. 3.2 of main manuscript\;
		X$^\text{corr}_\text{pbcc} \leftarrow$ $\emptyset$ \;
		\ForEach{x in X$_\text{pbcc}$}{
			\textbf{op} $\sim \mathcal{O}$ \tcp*{Sample Corruptions}  
			\textbf{sev} $\sim \mathcal{S}$ \tcp*{Sample Severity}
			$x_\text{corr} \leftarrow \psi$($x$, \textbf{op}, \textbf{sev})~\cite{hendrycks2018benchmarking} \tcp{Augments $x$ with corruption \textbf{op} of severity \textbf{sev}}
			$X^\text{corr}_\text{pbcc} \leftarrow$ \{X$^\text{corr}_\text{pbcc} \cup x_\text{corr}$\}\;
		}\;
		\KwRet X$^{corr}_{pbcc}$ 
	}
	
	\For{t = 1, 2, $\cdots$, m}{ \tcp{Training Loop}
		\ForEach{ $data$  in $\D^\text{train}_\text{in}$}{          \tcc{$data =$ (image, label)}
			X$_{ID}, \Y$ = $data$ \tcp*{X$_{ID}$ represents a batch of ID images} \;
			X$^\text{corr}_\text{pbcc}$ = \FSum{X$_{ID}$}\;
			$\mathbf{\mathcal{L}}$ = $\lce$(X$_{ID}, \Y$;$f_{\theta}^+$) + $\lce$(X$^\text{corr}_\text{pbcc}$, $K$+1;$f_{\theta}^+$)\;  
			% Train $\hat{f_{\theta}}$ for one iteration.
			Update model parameters $\theta$
		}
		
	}
	%
	\caption{Compounded Corruptions (CnC)}
	%
	\label{alg:cnc}
	%
\end{algorithm}

% PBCC(X_i,X_j)
% lam = np.random.beta(1,1)
% rand_index = torch.randperm(points.size()[0])   
% new_points = lam * points + (1. - lam) * points[rand_index]


==> scratchpad.tex <==
\begin{algorithm}[t]
	%\algsetup{linenosize=\tiny}
	\scriptsize %\small, \footnotesize, \scriptsize, or \tiny
	\label{algo_Rasha}
	\SetKwInput{KwInput}{Inputs}                % Set the Input
	\SetKwInput{KwOutput}{Output}  
	\SetKwInput{KwLoss}{Loss}  
	\DontPrintSemicolon
	\LinesNotNumbered
	\KwInput{
		$\D^\text{train}_\text{in}$  \tcp*{Train Set} 
		${f_{\theta}^+}$, $m$  \tcp*{Model, Number of epochs}
		$\mathcal{O}$ = \{contrast, $\cdots$, frost\} \tcp*{Corruption set}
		$\mathcal{S}$ = \{1, 2, 3, 4, 5\} \tcp*{Severity}
		$K+1$ \tcp*{Number of Classes}
	}
	\KwOutput{Trained Model $F^+$}
	%\tcp{\ood Data Generation}
	\SetKwFunction{FSum}{CnCDataGen} %\tcp*{\ood Data Generation} 
	
	\SetKwProg{Fn}{Function}{}{}
	\Fn{\FSum{X$_{ID}$}}{
		X$_\text{pbcc} \leftarrow$ Apply PBCC on X$_{ID}$\;
		X$^\text{corr}_\text{pbcc} \leftarrow$ $\emptyset$ \;
		\ForEach{x in X$_\text{pbcc}$}{
			\textbf{op} $\sim \mathcal{O}$ \tcp*{Sample Corruptions}  
			\textbf{sev} $\sim \mathcal{S}$ \tcp*{Sample Severity}
			$x_\text{corr} \leftarrow \psi$($x$, \textbf{op}, \textbf{sev})~\cite{hendrycks2018benchmarking} \tcp{Augments $x$ with corruption \textbf{op} of severity \textbf{sev}}
			$X^\text{corr}_\text{pbcc} \leftarrow$ \{X$^\text{corr}_\text{pbcc} \cup x_\text{corr}$\}\;
		}\;
		\KwRet X$^{corr}_{cmix}$ 
	}
	
	\For{t = 1, 2, $\cdots$, m}{ \tcp{Training Loop}
		\ForEach{ $data$  in $\D^\text{train}_\text{in}$}{          \tcc{$data =$ (image, label)}
			X$_{ID}, \Y$ = $data$\; \tcp{X$_{ID}$ is ID images}
			X$^\text{corr}_\text{cmix}$ = \FSum{X$_{ID}$}\;
			$\mathbf{\mathcal{L}}$ = $\lce$(X$_{ID}, \Y$;$f_{\theta}^+$) + $\lce$(X$^\text{corr}_\text{cmix}$, $K$+1;$f_{\theta}^+$)\;  
			% Train $\hat{f_{\theta}}$ for one iteration.
			Update model parameters $\theta$
		}
		
	}
	%
	\caption{Compounded Corruptions (CnC)}
	%
	\label{alg:cnc}
	%
\end{algorithm}



\mypara{Visualization of \id-\oods Separation}
%
\cref{fig:godinvscnc} shows the separation between \ids and \oods samples based on the scores given to them by CnC and Generalized-ODIN~\cite{hsu2020generalized}. For the experiment, \ids dataset is CIFAR-100 and \oods dataset is SVHN. For CnC we use the output probability for the $\text{(K+1)}^\text{th}$ class as the \oods score. The histogram obtained by plotting the \oods score for various samples from \ids and \oods dataset is shown in \cref{fig:godinvscnc}. Note that lesser the overlap, better the separation. % No overlap would imply perfect \oods and \ids separation, and is closely approximated by CnC. 
Plots for more \id-\oods combinations are in supplementary.
%Ideally, no overlap would imply perfect \oods and \ids separation which is almost achieved by CnC. We give plots for more combinations of \id-\oods datasets in the supplementary.

\begin{table}[t]
\small
	%\centering
	\setlength\tabcolsep{10pt}
	\begin{tabular}{ccccc}
		\toprule[1pt]
		\multirow{2}{*}{$\mathcal{D}_\text{in}^\text{train}$} & 
		\multicolumn{2}{c}{RMS CE $\downarrow$} & 
		\multicolumn{2}{c}{ECE $\downarrow$}
		\\ \cmidrule{2-5}
		& TS & CnC & TS & CnC 
		\\
		\midrule[0.75pt]
		CIFAR-10 & 11.1 & \textbf{6.2} & 5.1 & \textbf{3.2}
		\\
		CIFAR-100 & 26.1 & \textbf{19.3} & 19.6 & \textbf{15.4}
		\\
		\bottomrule[1pt]
	\end{tabular}
	\caption{Training with CnC data also leads to better calibration. Above, we compare the calibration errors of a model trained using \ids and our data, with the one which is trained only using \ids data and calibrated with temperature scaling (TS) \cite{guo2017calibration}.}
	\label{tab:CalE}
\end{table}




\begin{table}[t]
\scriptsize
\setlength\tabcolsep{3pt}%
\begin{center}
\resizebox{3cm}{!}{
\begin{tabular}{clccc}
\toprule
$\mathcal{D}_\text{out}^\text{test}$ & \textbf{\scriptsize{Method}} & \textbf{\scriptsize{TNR@95TPR}}& \textbf{\scriptsize{AUROC}} & \textbf{\scriptsize{DetErr}}
\\ 
%& & $\pmb{\uparrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ 

\midrule
\multirow{4}{*}{$\mathbf{TINc}$} & CutMix  & 93.7 & 98.7 & 5.4  \\
& Corruption  & 96.7 & 99.2 & 4.0  \\
& r-CnC  & 94.8 & 98.7 & 4.5  \\
& \textbf{CnC} & \textbf{99.7} & \textbf{99.9} & \textbf{1.3}  \\
\midrule
\multirow{4}{*}{$\mathbf{LSUNc}$} & CutMix  & 67.2 & 90.3 & 18.6  \\
& Corruption  & 96.7 & 99.2 & 4.1  \\
& r-CnC  & 95.4 & 98.7 & 5.9  \\
& \textbf{CnC} & \textbf{98.3} & \textbf{99.6} & \textbf{3.1}  \\
\midrule
\multirow{4}{*}{$\mathbf{SVHN}$} & CutMix  & 10.4 & 72.2 & 32.6  \\
& Corruption  & 98.5 & 99.5 & 2.8  \\
& r-CnC  & 98.0 & 98.5 & 10.8  \\
& \textbf{CnC} & \textbf{98.7} & \textbf{99.7} & \textbf{2.0}  \\
\bottomrule
\vspace{-0.8cm}
\end{tabular}
}
\end{center}
\caption{Ablation: We use CIFAR-100 as ID dataset and use DenseNet as network architecture for all methods. CnC denotes our proposed method CompoundedCorruptions and r-CnC denotes CutMixOverCorruption. For table see supplementary.}%Table~\ref{tab:ablation_complete}.}
\label{tab:ablation1}
\end{table}

%\vspace{-1em}








\begin{figure}[t]
	\begin{center}
		\includegraphics[width= 0.7\linewidth]{figs-main/godinvscnc.pdf}
		\caption{\small{\textcolor{red}{Histogram of \oods score given by CnC (K+1 classifier) and Generalized-ODIN \cite{hsu2020generalized}, a K class classifier based \oods detector, for CIFAR-100 as \id, and SVHN as the \oods dataset. We note that almost perfect separation is achieved by CnC with minimal overlap in the \id \oods sample scores.}}}
		\label{fig:godinvscnc}
	\end{center}
\end{figure}

























\mypara{Linearity argument from rebuttal}

For empirical validation, see t-SNE visualisation in Fig.~2 of main manuscript and a closeup  in Fig.~2 of Suppl. We also confirm the hypothesis through measurements in feature space using UMAP. We setup an experiment with two images belonging to two distinct classes from CIFAR10, then generate 10 CutMix samples for each value of $\mathbold{\lambda} \in \{0.1,0.2,\cdots,0.9\}$, where $\mathbold{\lambda}$ is combination ratio, and then for a fixed $\mathbold{\lambda}$ we calculate the mean euclidean distance between a) UMAP embedding of the CutMix generated image and b) $\mathbold{\lambda}$ weighted sum of the UMAP embedding of the two original images. The Table below shows the results:
\begin{center}
\setlength{\tabcolsep}{0.5\tabcolsep}
\begin{tabular}{|c|r|r|r|r|r|r|r|r|r|}
\hline
%& \multicolumn{9}{c|}{$\lambda$(Combination Ratio)} \\
%\cline{2-10}
$\mathbold{\lambda}$& 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & 0.8 & 0.9\\
\hline
Mean Dist. & 1.3 & 2.8 & 3.5 & 3.2 & 5.4 & 4.9 & 3.7 & 2.5 & 1.1\\
\hline
\end{tabular}
\end{center}
\vspace{-0.2cm}
We further find that the euclidean distance between the embeddings of two original(ID) images is 19.6, while the maximum deviation is $5.45$, which indicate that embeddings of the CutMix generated samples are approximately convex combination of original embeddings with minimal deviation.


\mypara{Integrated with main tables}

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{0.2\tabcolsep}
\begin{tabular}{l|cc|cc}
\hline
 & \multicolumn{2}{c|}{\scriptsize{$\mathcal{D}_\text{in}^\text{train}$(CIFAR-10)}} & \multicolumn{2}{c}{\scriptsize{$\mathcal{D}_\text{in}^\text{train}$(CIFAR-100)}} \\
\hline
\multirow{1}{*}{\textbf{\scriptsize{Method}}} & \scriptsize{TNR@TPR95} & \scriptsize{AUROC} & \scriptsize{TNR@TPR95} & \scriptsize{AUROC}
%\\ 
%& & $\pmb{\uparrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$  
\\ 
\hline
OE~\cite{hendrycks2018deep}  & 98.84 & 99.37 & 55.74 & 88.94 
\\
SOFL\cite{Mohseni_Pitale_Yadawa_Wang_2020}  & 98.71 & 99.34  & 64.34 & 93.09 \\
CnC(Proposed) & \textbf{99.85} & \textbf{99.95} & \textbf{99.12} & \textbf{99.78} \\
\hline
%\cline{2-6}
%\cline{2-6}
CnRE & 37.98 & 71.65  & - & -\\
CnRc &  98.43  &  99.51   & - & -\\
%\hline
%\multirow{3}{*}{\begin{turn}{90}\scriptsize CIFAR100\end{turn}} 
%& OE~\cite{hendrycks2018deep}  & 55.74 & 88.94 
%\\
%& SOFL\cite{Mohseni_Pitale_Yadawa_Wang_2020}  & 64.34 & 93.09 \\
%& CnC(Proposed) & \textbf{99.12} & \textbf{99.78} \\
%\hline
%\multirow{3}{*}{\begin{turn}{90}\scriptsize SVHN\end{turn}} 
%& OE~\cite{hendrycks2018deep}  & 99.8 & 99.97 
%& SOFL\cite{Mohseni_Pitale_Yadawa_Wang_2020}  & \textbf{99.99} & \textbf{99.99} \\
%& CnC(Proposed) & 99.2 & 99.9\\
\hline
\end{tabular}
\vspace{-0.5em}
\caption{\small{Comparison of \oods detectors. We use DenseNet-BC as feature extractor for all methods. The values are averaged over \oods datasets- LSUNc, LSUNr, iSUN, SVHN.}}
\label{tab:sota_comparison}
 \vspace{-2em}
\end{table}

%Thulasidasan \etal augment the training set with MixUp samples in a K class setting with soft targets unlike us with an explicit reject class. We have used Ref[3] for comparison. \textcolor{red}{(\#3)} Natural corruptions simulate OOD samples with non-semantic drift and we are not aware of any obvious way to do it in feature space. \textcolor{red}{(\#4)}) See Line 782: ``Detecting Domain Shift as OOD" in main manuscript \& Sec.~5 in Suppl. for results of suggested experiments. Despite plethora of OOD detectors available, we offer a simple technique with SOTA performance.












































\begin{table}
\begin{tabularx}{\linewidth}{@{}YYYY@{}}
%\label{tab:ablation} 


\toprule
  $\mathbf{Method}$ & $\mathbf{TNR}$ & $\mathbf{AUROC}$ & $\mathbf{DetErr}$\\ %& $\mathbf{AUPR In}$ & $\mathbf{AUPR Out}$ \\

  & $\mathbf{(95\% TPR)}$ & & \\
   & $\pmb{\uparrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ \\ % & \uparrow & \uparrow  \\
 \midrule
  CnC-2 & 86.3 & 89.5 & 29.2\\
  CnC-3  & 95.5 & 98.9 & 4.6  \\
  CnC-Gaussian  & 12.8 & 54.1 & 32.5  \\
  CnC & \textbf{99.3} & \textbf{99.8} & \textbf{1.7}  \\
 \hline
 \end{tabularx}
 \captionof{table}{Comparison between CnC, CnC-2, CnC-3, CnC-Gaussian. CnC refers to our proposed method which includes training using all 19 types of corruptions. CnC-2 refers to training using \texttt{snow} and \texttt{brightness}. CnC-3 refers to training using only a subset of corruptions which includes \texttt{contrast}, \texttt{saturate} and \texttt{frost}. CnC-Gaussian uses \texttt{Gaussian Blur} for corruptions. For all experiments we take a CIFAR-100 classifier and use DenseNet as feature extractor. The values are averaged over all \oods benchmark datasets.} %$\pmb{\uparrow}$ indicates larger value is better, and $\pmb{\downarrow}$ indicates lower value is better. All values are percentages. Bold numbers are superior results.}
 \label{tab:ablation3}
 \end{table}


In Supplementary Figure~\ref{fig:js-div}, we compute JS-Divergence metric between proxy \oods data generated by applying individual corruption types mentioned in \cite{hendrycks2018benchmarking} over CutMix~\cite{yun2019cutmix} generated images and CIFAR-100 training set. Since, low divergence score indicates higher similarity and vice-versa, we try to pick up corruptions which matches our constraint of generating samples both near and far from the boundary region, without digging deeper in ID manifold. From Supplementary Figure~\ref{fig:js-div}, we find that \texttt{snow} and \texttt{brightness} has lowest JS-Divergence score, hence applying these corruptions over CutMix~\cite{yun2019cutmix} would generate data that is most similar to original training set. However, that also signifies that the data generated using these corruptions, would more or less lie over the ID manifold and without spanning areas far from the boundary. We refer this type of training as CnC-2 (using 2 types of corruptions). 

 To investigate the significance of corruptions having high JS-Divergence score, we pick up \texttt{Gaussian Blur}, which generates proxy \oods samples most dissimilar to training data (Refer Suppl. Figure~\ref{fig:js-div}). We refer to this type of training as CnC-Gaussian.
 
 In Table~\ref{tab:ablation3}, we compare our proposed method with the variants obtained by training using various subsets of corruptions. We find that model trained using proxy \oods having both very low and high JS-Divergence scores renders useless. However, using subset of corruptions (\texttt{contrast}, \texttt{saturate} and \texttt{frost}) which generate samples both near and far from boundary is more useful.
 
 %Based on JS divergence score, we find that instead of training with the whole set of $19$ corruptions, proxy \oods data generated using only $3$ types of corruptions (\texttt{contrast}, \texttt{saturate} and \texttt{frost}) can attain almost same \oods detection performance as originally proposed CnC% trained using whole set of corruptions mentioned in \cite{hendrycks2018benchmarking}. 
 %However, this is only a single combination out of several possible combinations of corruptions and we are still in process of finding the subset of corruptions which matters the most for ID-\oods separation. We denote this method of generating proxy \oods data as CnC-3 (using 3 types of corruptions). In Table~\ref{tab:ablation3}, we compare our proposed method with the variants obtained by training using various subsets of corruptions.



%we have ${K \choose 2}$ binary discriminant functions, one for every possible pair of classes. So, OOD class comprises of ${K \choose 2}$ generated points (it could be ${K \choose 2}$*75 based on corruption severity/degree. We conjecture that generated points that are in between decision surface matter to the classification process and a random data point very far away in embedding space does not appeal to the classifier's decision making process. CnC generates the points in between the classes and there could be the points that lie outside these classes like a Gaussian noise/Uniform noise images. In a nutshell, we are increasing the sample space of OOD points in the following way:  use CutMix generated datapoints; then applying corruptions of various degree/types to create an epsilon ball around every CutMix point and then apply standard gradient descent to learn better.}

 
 
%\ramya{Updated: Using training data, DNN carves out the embedding space into decision regions i.e., $K+1$ classes in our case. We are interested to generate the samples close to and far from the boundary for our $K+1^{th}$ class. In order to do so, we perform cutMix to generate synthetic samples which spans the region between the two class. Then we perform corruptions as described below which would redistribute the points around the epsilon radii ball and some of the points lie on cluster boundary. Since, we perform \emph{CorruptionOverCutMix} we would inherit the properties of CutMix which we believe can generate points that span the non decision regions b/w a pair of clusters dipicted in grey.} 

%\ramya{Unfortunately failing: To demonstrate why we think CnC is better than CutMix, we hypothesise training using a minibatch of just CutMix points and then CnC points should result in different gradients at a particulat layer: Will CutMix gradients be close to zero using cutmix points but not cnc points. If gradients are positive then we could be learning better using CnC points.}

%we find that CutMix images between two classes usually lies in the feature space between the two classes depending on proportion of patches extracted.
%\ramya{the notion of radii ball and specifically episilon is missing in all the equations, Need to include some reference}


\begin{figure*}
\label{fig:js}
\begin{center}
\includegraphics[width = 0.95\linewidth]{js-div.png}
%\fcolorbox{black}{black}{\includegraphics[scale=0.25]{}}
\caption{To study the effect of individual corruption type, we plot the histogram of JS-Divergence scores computed between training set images(CIFAR-100) and proxy \oods data generated by applying individual corruptions mentioned in \cite{hendrycks2018benchmarking} over CutMix~\cite{yun2019cutmix} generated images.}
\label{fig:js-div}
\end{center}
\end{figure*}

 
\noindent\setlength\tabcolsep{6pt}%


\begin{table}[t]
 \centering
 \resizebox{0.7\linewidth}{!}{%

 
 
 \begin{tabular}{l|ll|ccc}
\toprule
 $\mathcal{D}_{in}^{train}$ & $\mathcal{D}_{out}^{test}$ & $\mathbf{Method}$ & $\mathbf{TNR}$ & $\mathbf{AUROC}$ & $\mathbf{DetErr}$\\ %& $\mathbf{AUPR In}$ & $\mathbf{AUPR Out}$ \\
 
  & & & $\mathbf{(95\% TPR)}$ & & \\
  & & & $\pmb{\uparrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$  \\ % & \uparrow & \uparrow  \\
 \cline{2-6}
 \multirow{54}{*}{\begin{turn}{90}$\mathbf{CIFAR-100}$\end{turn}} & \multirow{9}{*}{$\mathbf{TINc}$} & Mixup (ICLR'18) \cite{zhang2017mixup}  & 29.3 & 79.1 & 28.6  \\
& & CutOut (arXiV,17) \cite{devries2017improved} & 66.2 & 93.4 & 14.0  \\
& & CutMix (ICCV'19) \cite{yun2019cutmix} & 93.7 & 98.7 & 5.4    \\
& & GridMask (arXiV'20) \cite{chen2020gridmask} & 18.6 & 74.6 & 30.6  \\
& & SaliencyMix (ICLR'21) \cite{uddin2021saliencymix} & 96.3  & 99.3 & 3.7 \\
& & AugMix (ICLR'20) \cite{hendrycks*2020augmix} & 56.5 & 86.9 & 17.3 \\
& & RandomErase (AAAI'20) \cite{zhong2017random} & 14.9 & 71.2 & 32.7 \\
& & Corruptions (ICLR'19) \cite{hendrycks2018benchmarking} & 96.7 & 99.2 & 4.0 \\
& & PuzzleMix (ICML'20) \cite{kim2020puzzle} & 71.4 & 92.7 & 15.2 \\
& & RandAugment (NeurIPS'20) \cite{RandAugment} & 98.7 & 99.7 & 2.2 \\
& & SuperMix (CVPR'21) \cite{dabouei2020supermix} & 48.5 & 90.5 & 17.2\\
& & Fmix (ICLR'21) \cite{harris2021fmix} & 72.3 & 94.2 & 14.2\\
& & Noise & 53.0 & 91.2 & 16.9 \\
& & \textbf{CnC(Proposed)} & \textbf{99.7} & \textbf{99.9} & \textbf{1.3}\\
 \cline{2-6}
& \multirow{9}{*}{$\mathbf{TINr}$} & Mixup (ICLR'18) \cite{zhang2017mixup}  & 34.4 & 70.9 & 15.0  \\
& & CutOut (arXiV,17) \cite{devries2017improved} & 71.8 & 94.8 & 12.0  \\
& & CutMix (ICCV'19) \cite{yun2019cutmix} & 91.0 & 98.3 & 6.9    \\
& & GridMask (arXiV'20) \cite{chen2020gridmask} & 15.1 & 72.7 & 32.1  \\
& & SaliencyMix (ICLR'21) \cite{uddin2021saliencymix} & 96.2  & 99.3 & 4.0 \\
& & AugMix (ICLR'20) \cite{hendrycks*2020augmix} & 54.4 & 86.4 & 17.8 \\
& & RandomErase (AAAI'20) \cite{zhong2017random} & 15.1 & 72.0 & 32.2 \\
& & Corruptions (ICLR'19) \cite{hendrycks2018benchmarking} & 94.5 & 98.9 & 5.0 \\
& & PuzzleMix (ICML'20) \cite{kim2020puzzle} & 77.8 & 94.4 & 12.9\\
& & RandAugment (NeurIPS'20) \cite{RandAugment} & \textbf{99.7} & \textbf{99.9} & \textbf{1.0} \\
& & SuperMix (CVPR'21) \cite{dabouei2020supermix} & 40.3 & 89.2 & 18.2 \\
& & Fmix (ICLR'21) \cite{harris2021fmix} & 79.5 & 95.7 & 11.7\\
& & Noise & 55.3 & 91.8 & 16.0\\
& & \textbf{CnC(Proposed)} & 99.6 & 99.8 & 1.6\\
 \cline{2-6}
 & \multirow{9}{*}{$\mathbf{LSUNc}$} & Mixup (ICLR'18) \cite{zhang2017mixup}  & 51.2 & 89.1 & 19.7  \\
& & CutOut (arXiV,17) \cite{devries2017improved} & 25.3 & 77.4 & 30.1  \\
& & CutMix (ICCV'19) \cite{yun2019cutmix} & 67.2 & 90.3 & 18.6   \\
& & GridMask (arXiV'20) \cite{chen2020gridmask} & 16.3 & 70.9 & 33.7  \\
& & SaliencyMix (ICLR'21) \cite{uddin2021saliencymix} & 68.2  & 91.4 & 18.1 \\
& & AugMix (ICLR'20) \cite{hendrycks*2020augmix} & 65.5 & 89.6 & 13.8 \\
& & RandomErase (AAAI'20) \cite{zhong2017random} & 9.9 & 63.9 & 38.7\\
& & Corruptions (ICLR'19) \cite{hendrycks2018benchmarking} & 96.7 & 99.2 & 4.1 \\
& & PuzzleMix (ICML'20) \cite{kim2020puzzle} & 63.8 & 89.0 & 19.9 \\
& & RandAugment (NeurIPS'20) \cite{RandAugment} & 78.1 & 95.6 & 12.6 \\
& & SuperMix (CVPR'21) \cite{dabouei2020supermix} & 53.5 & 90.0 & 18.2 \\
& & Fmix (ICLR'21) \cite{harris2021fmix} & 20.9 & 78.5 & 27.5\\
& & Noise & 35.6 & 85.2 & 23.1\\
& & \textbf{CnC(Proposed)} & \textbf{98.3} & \textbf{99.6} & \textbf{3.1}\\
 \cline{2-6}
 & \multirow{9}{*}{$\mathbf{LSUNr}$} & Mixup (ICLR'18) \cite{zhang2017mixup}  & 35.8 & 67.9 & 10.4  \\
& & CutOut (arXiV,17) \cite{devries2017improved} & 73.2 & 95.5 & 10.5  \\
& & CutMix (ICCV'19) \cite{yun2019cutmix} & 97.2 & 99.4 & 3.4 \\
& & GridMask (arXiV'20) \cite{chen2020gridmask} & 22.0 & 79.4 & 26.7  \\
& & SaliencyMix (ICLR'21) \cite{uddin2021saliencymix} & 98.9 & 99.8 & 1.9 \\
& & AugMix (ICLR'20) \cite{hendrycks*2020augmix} & 47.0 & 84.2 & 20.7 \\
& & RandomErase (AAAI'20) \cite{zhong2017random} & 15.3 & 70.6 & 32.9\\
& & Corruptions (ICLR'19) \cite{hendrycks2018benchmarking} & 95.7 & 99.1 & 4.5 \\
& & PuzzleMix (ICML'20) \cite{kim2020puzzle} & 86.4 & 97.0 & 9.1\\
& & RandAugment (NeurIPS'20) \cite{RandAugment} & \textbf{99.9} & \textbf{100.0} & \textbf{0.5} \\  %% tHIS IS HIGHEST
& & SuperMix (CVPR'21) \cite{dabouei2020supermix} & 52.2 & 92.3 & 14.4 \\
& & Fmix (ICLR'21) \cite{harris2021fmix} & 83.7 & 96.5 & 10.2\\
& & Noise & 64.3 & 94.0 & 13.2\\
& & \textbf{CnC(Proposed)} & \textbf{99.9} & 99.9 & 0.9\\
 \cline{2-6}
 & \multirow{9}{*}{$\mathbf{iSUN}$} & Mixup (ICLR'18) \cite{zhang2017mixup}  & 35.0 & 69.4 & 10.4  \\
& & CutOut (arXiV,17) \cite{devries2017improved} & 65.7 & 93.8 & 13.0  \\
& & CutMix (ICCV'19) \cite{yun2019cutmix} & 95.2 & 99 & 4.8    \\
& & GridMask (arXiV'20) \cite{chen2020gridmask} & 21.0 & 78.8 & 27.4  \\
& & SaliencyMix (ICLR'21) \cite{uddin2021saliencymix} & 97.9  & 99.6 & 2.8 \\
& & AugMix (ICLR'20) \cite{hendrycks*2020augmix} & 55.4 & 88.1 & 16.7 \\
& & RandomErase (AAAI'20) \cite{zhong2017random} & 16.4 & 71.5 & 32.4 \\
& & Corruptions (ICLR'19) \cite{hendrycks2018benchmarking} & 94.0 & 98.8 & 5.3 \\
& & PuzzleMix (ICML'20) \cite{kim2020puzzle} & 83.6 & 96.3 & 10.2\\
& & RandAugment (NeurIPS'20) \cite{RandAugment} & 99.4 & 99.8 & \textbf{1.2} \\
& & SuperMix (CVPR'21) \cite{dabouei2020supermix} & 44.7 & 90.3 & 16.8 \\
& & Fmix (ICLR'21) \cite{harris2021fmix} & 80.1 & 95.6 & 11.8\\
& & Noise & 56.9 & 92.2 & 15.5 \\
& & \textbf{CnC(Proposed)} & \textbf{99.6} & \textbf{99.9} & 1.4\\
 \cline{2-6}
 & \multirow{9}{*}{$\mathbf{SVHN}$} & Mixup (ICLR'18) \cite{zhang2017mixup}  & 25.1 & 83.5 & 25.3  \\
& & CutOut (arXiV,17) \cite{devries2017improved} & 38.5 & 67.9 & 4.8  \\
& & CutMix (ICCV'19) \cite{yun2019cutmix} & 10.4 & 72.2 & 32.6   \\
& & GridMask (arXiV'20) \cite{chen2020gridmask} & 13.5 & 75.2 & 29.5  \\
& & SaliencyMix (ICLR'21) \cite{uddin2021saliencymix} & 20.6  & 83.8 & 22.3 \\
& & AugMix (ICLR'20) \cite{hendrycks*2020augmix} & 29.9 & 83.3 & 22.5 \\
& & RandomErase (AAAI'20) \cite{zhong2017random} & 4.7 & 61.5 & 39.6\\
& & Corruptions (ICLR'19) \cite{hendrycks2018benchmarking} & 98.5 & 99.5 & 2.8 \\
& & PuzzleMix (ICML'20) \cite{kim2020puzzle} & 16.3 & 78.4 & 27.5 \\
& & RandAugment (NeurIPS'20) \cite{RandAugment} & 17.0 & 74.4 & 31.8 \\
& & SuperMix (CVPR'21) \cite{dabouei2020supermix} & 22.5 & 83.5 & 25.2 \\
& & Fmix (arxiv'21) \cite{harris2021fmix} & 11.7 & 75.6 & 29.4\\
& & Noise & 7.5 & 66.4 & 39.2\\
& & \textbf{CnC(Proposed)} & \textbf{98.7} & \textbf{99.7} & \textbf{2.0}\\
 %\cline{2-6}
\bottomrule
\end{tabular}
}
\caption{Comparison of Data Synthesis Methods for OOD detection when ID dataset is CIFAR100 (Note: main manuscript Table 3 provided results when CIFAR10 was considered as ID dataset). We use DenseNet as network architecture for all methods.}
% $\pmb{\uparrow}$ indicates larger value is better, and $\pmb{\downarrow}$ indicates lower value is better. All values are percentages.
\label{tab:c100_data_aug}
%\end{center}
\end{table}

==> sections/abstract.tex <==

%  \textcolor{blue}{in-distribution accuracy}\soumya{I think this can be bit of an overclaim, because our main focus is not on ID acc.},

==> tables/fig-polytope.tex <==
\begin{comment}
    
\begin{figure}[t]
	\def\imgwidth{\linewidth}
	\centering
	\begin{subfigure}
	%[Training Data]
		\centering
		\includegraphics[width=0.32\textwidth]{figs-main/polytopes/train_data-2.pdf}  
		%\caption{{\tiny Training Data}}
	\end{subfigure}
	\hfill
	\begin{subfigure}
	%[Vanilla]
		\centering
		\includegraphics[width=0.32\linewidth]{figs-main/polytopes/vanilla_32.pdf}  
		%\caption{Vanilla}
	\end{subfigure}
	\hfill
	\begin{subfigure}
	%[PBCC]
		\centering
		\includegraphics[width=0.32\linewidth]{figs-main/polytopes/cutmix_32.pdf}  
		%\caption{PBCC}
	\end{subfigure}
\\
	\begin{subfigure}
	%[Corruption]
		\centering
		\includegraphics[width=0.32\linewidth]{figs-main/polytopes/corr_32.pdf}  
		%\caption{Corruption}
	\end{subfigure}
	\hfill
	\begin{subfigure}
	%[r-CnC]
		\centering
		\includegraphics[width=0.32\linewidth]{figs-main/polytopes/rcnc_32.pdf}  
		%\caption{r-CnC}
	\end{subfigure}
	%\caption{$y=5/x$}
	\begin{subfigure}
		\centering
		\includegraphics[width=0.32\linewidth]{figs-main/polytopes/cnc_32.pdf}  
		%\caption{CnC}
	\end{subfigure}
	\caption{Visualization of trained classifiers as a result of \ood augmentation. A ReLU type \dnn is trained on the two-dimensional half-moon data set. The shattered neural networks \cite{hein2019relu} show that CnC has the tightest fit around the ID regions, as measured by the area of the (white colored) polytopes in which no training \id point is observed but a network predicts a point in that region as \id. The measured areas for such polytopes are \textbf{Vanilla training without data augmentation}:5.65,  \textbf{PBCC}: 8.20, \textbf{Corruption}:0.40,  \textbf{r-CnC}: 5.66, \textbf{CnC}: 0.37. Note that according to \cite{xuji} the more densely supported a polytope is by the training set, the more reliable the network is in that region. Hence, the samples declared \id in the regions where no \id sample is observed may actually be \ood with high probability. We observe that PBCC/r-CnC/Vanilla, all predict \id in many such polytopes. Recall that in r-CnC we reverse the order of PBCC and corruptions, i.e., we first apply corruptions over the input images followed by PBCC over the corrupted images.}% \textbf{See Suppl. for additional details.}}
		%Note: r-CnC is PBCC over Corruptions.}
	\label{fig:polytope}
\end{figure}
\end{comment}

==> tables/fig-umap.tex <==
\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{figs-main/toy.pdf}  

	\caption{An illustration of \ood synthesis on toy dataset with four \id classes: PBCC generates \ood points through a convex combination of ID points from different classes in $4 \choose 2$ ways, whereas corruptions can generate \ood points around each cluster. Observe that points generated by CnC spans wider \ood space including inter-ID-cluster area as well as outside the convex hull of \id points.} %We also provide a t-SNE/UMAP embedding visualisation in Supplementary. 
	\label{fig:umap}
\end{figure}


\begin{comment}
	\def\imgwidth{width=0.2\linewidth}
	\centering
	\begin{subfigure}{\imgwidth}
		\centering
		\includegraphics[width=0.2\linewidth]{figs-main/cnc_illustration/train_data.png}  
		\caption{\id}
	\end{subfigure}
	\begin{subfigure}{\imgwidth}
		\centering
		\includegraphics[width=0.2\linewidth]{figs-main/cnc_illustration/corr.png}  
		\caption{Corr}
	\end{subfigure}
	\begin{subfigure}{\imgwidth}
		\centering
		\includegraphics[width=0.2\linewidth]{figs-main/cnc_illustration/cutmix.png}  
		\caption{PBCC}
	\end{subfigure}
	\begin{subfigure}{\imgwidth}
		\centering
		\includegraphics[width=0.2\linewidth]{figs-main/cnc_illustration/rcnc.png}  
		\caption{r-CnC}
	\end{subfigure}
	\begin{subfigure}{\imgwidth}
		\centering
		\includegraphics[width=0.2\linewidth]{figs-main/cnc_illustration/cnc.png}  
		\caption{CnC}
	\end{subfigure}
	%\caption{UMAP \cite{mcinnes2018umap} embeddings of Corruptions, PBCC, and CnC. r-CnC refers to the method when the order of application of PBCC and corruptions are reversed (corrupt \id images then PBCC). Augmented \ood samples are depicted in \textcolor{red}{red}. The \id points are from CIFAR-10 with DenseNet feature extractor. While Corruption samples are primarily located on top of \id clusters, PBCC are mostly in the inter-\id space. CnC manages to sample both near and far regions more uniformly. }
	\begin{subfigure}{\imgwidth}
		\centering
		\includegraphics[width=\linewidth]{figs-main/UMAP-ID-1.pdf}  
		\caption{\id}
	\end{subfigure}
	\begin{subfigure}{\imgwidth}
		\centering
		\includegraphics[width=\linewidth]{figs-main/UMAP-Corr-1.pdf}  
		\caption{Corr}
	\end{subfigure}
	\begin{subfigure}{\imgwidth}
		\centering
		\includegraphics[width=\linewidth]{figs-main/UMAP-CutMix-1.pdf}  
		\caption{PBCC}
	\end{subfigure}
	\begin{subfigure}{\imgwidth}
		\centering
		\includegraphics[width=\linewidth]{figs-main/polytopes/UMAP_r-CnC_rasha.pdf}  
		\caption{r-CnC}
	\end{subfigure}
	\begin{subfigure}{\imgwidth}
		\centering
		\includegraphics[width=\linewidth]{figs-main/UMAP-CnC-1.pdf}  
		\caption{CnC}
	\end{subfigure}
\end{comment}

==> tables/id_test_acc.tex <==
\noindent\setlength\tabcolsep{6pt}%
%\begin{center}
\begin{table}
\begin{tabularx}{\linewidth}{@{}lYYYY@{}}
%\label{tab:ablation}
%\begin{tabularx}{\linewidth}{lc*{5}{>{\arraybackslash}X}}
%\begin{center}
% \label{tab:ablation1}
 \toprule
 $\mathcal{D}_{in}^{train}$ & Model & Baseline & CnC & Corr\\ %& $\mathbf{AUPR In}$ & $\mathbf{AUPR Out}$ \\
 \midrule
 CIFAR -10 & DenseNet & 95.3$\pm$0.1 & 94.63$\pm$0.51 & 93.8$\pm$0.1 \\
 CIFAR -100 & DenseNet & 77.8$\pm$0.1 & 76.8$\pm$0.92 & 76.6$\pm$0.1 \\
 SVHN & DenseNet & 98.1$\pm$0.1 & 97.9$\pm$0.1 & 97.6$\pm$0.1 \\
%  CIFAR -10 & ResNet & 94.4$\pm$0.1 & 93.9$\pm$0.1 & 92.3$\pm$0.1 \\
%  CIFAR -100 & ResNet & 76.2$\pm$0.1 & 76.2$\pm$0.1 & 75.4$\pm$0.1 \\
%  SVHN & ResNet & 96.9$\pm$0.1 & 96.9$\pm$0.1 & 96.4$\pm$0.1 \\
 CIFAR -10 & WideResNet & 94.3$\pm$0.26 & 94.33$\pm$0.21 & 94.2$\pm$0.31 \\
 CIFAR -100 & WideResNet  & 75.32$\pm$0.22 & 75.11$\pm$0.31 & 74.92$\pm$0.53 \\
 TinyImageNet & ResNet  & 57.0$\pm$0.21 & 60.5$\pm$0.59 & $\pm$- \\
\bottomrule

\end{tabularx}
\captionof{table}{Comparison of ID Test Accuracy. Baseline refers to standard training procedures. Training with only Corruptions reduces the test accuracy by % a significant 
margin.}
\label{tab:id_test_acc}
\end{table}

==> tables/table_calibration.tex <==
\begin{table}[t]
\small
\begin{center}
    

	%\resizebox{0.8\linewidth}{!}{%
		\begin{tabular}{ccccc}

			\toprule[1pt]
			\multirow{2}{*}{$\mathcal{D}_\text{in}^\text{train}$} & 
			\multicolumn{2}{c}{RMS CE $\downarrow$} & 
			\multicolumn{2}{c}{ECE $\downarrow$}
			\\ \cmidrule{2-5}
			& TS & CnC & TS & CnC 
			\\
			\midrule[0.75pt]
			CIFAR-10 & 11.1 & \textbf{6.2} & 5.1 & \textbf{3.2}
			\\
			CIFAR-100 & 26.1 & \textbf{19.3} & 19.6 & \textbf{15.4}
			\\
			\bottomrule[1pt]
		\end{tabular}%
		\end{center}
			 	\caption{\small CnC trained models are better calibrated as compared to models trained using Temperature Scaling.}
%	}
 	\label{tab:calib}
\end{table} 

